HyPFuzz: Formal-Assisted Processor Fuzzing

Recent research has shown that hardware fuzzers can effectively detect security vulnerabilities in modern processors. However, existing hardware fuzzers do not fuzz well the hard-to-reach design spaces. Consequently, these fuzzers cannot effectively fuzz security-critical control- and data-flow logic in the processors, hence missing security vulnerabilities. To tackle this challenge, we present HyPFuzz, a hybrid fuzzer that leverages formal verification tools to help fuzz the hard-to-reach part of the processors. To increase the effectiveness of HyPFuzz, we perform optimizations in time and space. First, we develop a scheduling strategy to prevent under- or over-utilization of the capabilities of formal tools and fuzzers. Second, we develop heuristic strategies to select points in the design space for the formal tool to target. We evaluate HyPFuzz on five widely-used open-source processors. HyPFuzz detected all the vulnerabilities detected by the most recent processor fuzzer and found three new vulnerabilities that were missed by previous extensive fuzzing and formal verification. This led to two new common vulnerabilities and exposures (CVE) entries. HyPFuzz also achieves 11.68$\times$ faster coverage than the most recent processor fuzzer.

==> openarch/implementation.tex <==
\section{Implementation}\label{sec:imp}
We implemented \ourtool{} to:
%While implementing \ourtool{}, we have three goals: 
(i) be compatible with industrial integrated circuit~(IC) design and verification flow, (ii) penetrate deep into the \nn{design-under-test}~(DUT) and explore it exhaustively to detect vulnerabilities, and (iii) identify uncovered points in the DUT given the branch coverage metric of \vcs{}, extract the logical conditions required to cover them, and convert these conditions into the properties that can be proven with formal tools. We describe the implementation of various components of \ourtool{} in this section. 


\textbf{Fuzzing Engine.}
\difuzz{}~\cite{hur2021difuzzrtl} and \thehuzz{}~\cite{kandethehuzz} are the \nn{most-recent} hardware fuzzing engines capable of fuzzing processor designs like \cva{}~\cite{cva6} and \rc{}~\cite{rocket_chip_generator}. 
%We consider \difuzz{}~\cite{hur2021difuzzrtl} and \thehuzz{}~\cite{kandethehuzz} as the most advanced hardware fuzzers because they verified multiple open-sourced processors, such as \cva{}~\cite{cva6} and \rc{}~\cite{rocket_chip_generator}, that are closed to the industrial-level designs and detected multiple vulnerabilities from them.
Among these, we picked \thehuzz{} as our fuzzing engine because: 
%We select \thehuzz{}~\cite{kandethehuzz} as the fuzzing engine of \ourtool{} for the following reasons: 
(i) the coverage metrics used by \thehuzz{} are hardware code-coverage metrics, widely used in the semiconductor industry and achieve faster code-coverage compared to \difuzz{}~\cite{kandethehuzz},
(ii) \thehuzz{} directly instruments any HDL while \difuzz{} requires converting the \verilog{} and \systemverilog{} designs to Chisel using open-source tools before they can be instrumented, and
%(i) \thehuzz{} is compatible with industrial hardware verification tools such as Synopsys \vcs{}~\cite{vcs} and Siemens \modelsim{}~\cite{modelsim}, to generate code coverage as feedback to guide its mutation algorithms. This makes it support designs in various HDLs. However, \difuzz{}~\cite{hur2021difuzzrtl} develops its own coverage metric; based on its open-sourced code, the strategy only supports designs written in Chisel~\cite{bachrach2012chisel}. 
(iii) \thehuzz{} directly mutates the binary executable inputs and hence supports even illegal instructions not recognized by the ISA compilers, on the other hand, \difuzz{} mutates assembly instructions and then compiles them to generate the binary executable; thus it cannot support illegal instructions in its input. 
%(2) The mutation can happen in two formats: source code and executable binary. \difuzz{}~\cite{hur2021difuzzrtl} mutates its test cases in source code and applies ISA specific compilers to generate executable binary. The compilers will filter out the test cases with illegal instructions that violate ISA reference. However, \thehuzz{}~\cite{kandethehuzz} mutates test cases in the binary format, allowing the appearance of illegal instructions, which introduces more chaos to designs and explores designs exhaustively, such as the illegal instruction handler in processors.
We provide the input programs generated by the \JG{} as seeds to \thehuzz{}, monitor the increase in coverage and fuzzing time, and terminate it based on the scheduling strategy. 


\textbf{Property Generator.}
%\subsection{Uncovered Point Selector}
We implemented the property generator in Python. \ourtool{} invokes it when \thehuzz{} is terminated by the scheduling strategy and before starting \JG{}. Property generator parses the coverage data from \thehuzz{} to identify the uncovered coverage points and invokes the selection strategy to select coverage points among these uncovered points.

Next, to extract the conditions required to cover these points, \ourtool{} traverses the control flow graph~(CFG) for each module of the DUT based on the branch statements in modules. The branch statement information is extracted by parsing the coverage data generated by the instrumentation logic of the \vcs{} simulator. 
All the branch coverage points now become leaf nodes in this CFG. The condition to cover the branch coverage points is the sequence of branch statements starting from the root node to the leaf node corresponding to that branch coverage point. These conditions are then converted to SVA properties and inserted in the DUT. 
%Property generator is the bridge that connects \thehuzz{}~\cite{kandethehuzz} and \JG{}~\cite{jaspergold}. It needs to take the coverage feedback of \thehuzz{}~\cite{kandethehuzz} as inputs, identifies and selects uncovered points from it, and converts the conditions of covering each point into a SVA property as outputs for \JG{} to find a trace. Because \ourtool{} specifically focuses on branch type coverage metrics, we will establish a control flow graph~(CFG) for each module in the design based on the branch statements and the location of coverage points in each module to identify the conditions of covering a point.  For example, \vcs{}'s branch metric allocates coverage points at leaf nodes of each CFG~\cite{vcs}; we need to include all branch statements from the root node to one leaf node as the conditions of covering the point at the leaf node. This process can be done by parsing the coverage report from \vcs{}~\cite{vcs}. 

As our property generator is using coverage data from the \vcs{} simulator, it is scalable to large hardware designs written in any HDLs. Note that the CFG is built only once at the start of \ourtool{} and reused every time we want to identify conditions of covering a point. We further reduce the overhead due to property generator by caching the properties it generates and reuse them directly if needed in the future.  
%More implementation details are included in the Appendix section~\ref{sec:appendix}. Because property generator is developed based on industrial tool's outputs, we believe the identification of uncovered points and their conditions is more reliable than methods using self-developed coverage metrics.


% \subsection{Formal Engine}
% The formal engine in \ourtool{} can be any hardware formal tool capable of proving \systemverilog{} assertions. 
% We used Cadence \JG{}~\cite{jaspergold} as the formal engine. \JG{} is a popular formal verification tool extensively used in the semiconductor industry. It supports various hardware description languages~(HDLs), such as \verilog{} and \systemverilog{}. 
% \JG{} is capable of scaling to large industrial-level IC designs and optimized for memory and time consumption\todo{need reference}. \todo{give example of a very large design that uses JG. it should be there on cadence website}. 
% The takes the DUT (with system verilog assertion~(SVA) constraints and properties added to it) as the input, proves the properties, and report if the property can be reached or not. The tool can dump trace data in case of reachable properties which consists of values of all the signals used to change the state of the DUT from initial state to triggering the property. 
% %The tool will receive DUT with constraints and properties in system verilog assertion~(SVA) format as inputs. Its proof process will identify if a property is reachable or not and can dump a trace for a reachable one. 
% %The trace contains the values of signals that lead a DUT from an initial state to the corresponding reachable property.

% \noindent \textbf{Constraining the environment}.
% %\subsection{Constraining the Environment of Formal Engine}
% When the DUT (processor) is simulated, it is enclosed in a SoC framework which generates the inputs to the processor (the input to the SoC itself is the binary executable we load into the main memory of the SoC). Thus, the input signals of the processor are not directly controlled by the test-bench during the simulation and restricted by the interface between the SoC and the processor.  
% But, when the DUT is loaded into the formal engine, by default, formal engine assumes that any value can be assigned to the input signals of the DUT. It is essential to inform the formal engine about the restrictions during simulation due to the SoC interface to ensure that the trace data generated by the formal tool can be accurately replicated during the fuzzer simulations.  
% %The stimuli from the formal engine may not cover the same points in simulation if we do not constrain the environment of it to be the same as simulation's. \JG{} will think that the inputs of DUT's top module are non-deterministic signals and can have any possible values if there is no constraints. However, the simulation environment of a processor usually contains multiple SoC peripherals~\cite{chipyard}, such as bus and memory, and the processor's inputs must follow the format of bus protocols. 
% Thus we constrain the environment of the formal tool to be the same as the environment of the simulation by:
% %so that we can obtain valid stimuli from \JG{}. To achieve this goal, we 
% (i) constraining the global configurations used during simulation. For example, the simulation of \cva{} disables the debug mode and interrupt behaviors from SoC peripherals; thus, we constrain the corresponding top module's inputs in the formal engine.
% %into the same behaviors. Then, we 
% (ii) constraining the initial state of DUT in formal engine so that it will start at the same initial state that in the simulation---\JG{} allows us to do this using a waveform from the simulation (\JG{} takes the values of all the flip-flops from a specified time in the waveform and sets the same as its initial state when proving properties). The time at which values are extracted from the waveform is the clock cycle in which the simulation starts executing the testing instructions.  
% %load an initial state from a simulation waveform which will clarify the values on all flip-flops at the initial state. This requires us to provide the location of the initial state in a waveform. Because the simulation of processor in \thehuzz{}~\cite{kandethehuzz} will always start from the same initial state before executing testing instructions, we observe the last cycle of initial state and load it with waveform to \JG{}.

\textbf{Seed Generator.}
Once \JG{} proves that the property of an uncovered point is reachable, it will generate a trace as a waveform showing a sequence of signals that can set a DUT into the target state. This state will fit the property and satisfy the conditions of covering the corresponding point. 
However, the trace cannot be directly used as seeds because \thehuzz{} uses a sequence of instructions in a binary format binary as inputs.  
%Once the formal process is done, each uncovered point will have its trace if the corresponding property is reachable. However, these traces can not be used as stimuli of \thehuzz{} directly because the format is different with the test cases of \thehuzz{}'s simulation environment. 
Therefore, we built a seed generator in Python to extract the sequence of instructions required to trigger the coverage points from the trace using an existing trace parser tool, and generate a binary executable consisting of these instructions as payload by replacing the dummy instructions in a pre-built template binary executable. 
The input to the trace parser tool is the trace data itself and the name of the signal(s) storing the instruction data. In processors, instruction data is typically stored in two signals: (i) instruction signal in the commit module, and (ii) instruction signal in the decoder module. We use the latter to ensure even the instructions causing exceptions or transient executions that are dropped before reaching the commit stage are included in the input generated by the seed generator. This ensures that the simulation of \thehuzz{} also runs the same sequence of instructions as the ones used by \JG{} to cover the coverage points. 
%need to extract the sequence of instructions from the trace so that \thehuzz{} uses them as a test case to cover the same point in simulation. There are two signals as candidates: (1) the signal that records instructions commited by a processor. (2) the instruction signal of decoder's input. Because the instructions causing exceptions or eliminated by branch mis-prediction will not get commited by a processor in general, we select the instruction signal of decoder's input to extract the sequence of instructions for each point as stimuli of \thehuzz{}.
